Composable Effects for Flexible and Accelerated Probabilistic Programming in NumPyro

NumPyro is a lightweight library that provides an alternate NumPy backend to the Pyro probabilistic programming language with the same modeling interface, language primitives and effect handling abstractions. Effect handlers allow Pyro's modeling API to be extended to NumPyro despite its being built atop a fundamentally different JAX-based functional backend. In this work, we demonstrate the power of composing Pyro's effect handlers with the program transformations that enable hardware acceleration, automatic differentiation, and vectorization in JAX. In particular, NumPyro provides an iterative formulation of the No-U-Turn Sampler (NUTS) that can be end-to-end JIT compiled, yielding an implementation that is much faster than existing alternatives in both the small and large dataset regimes.

==> nuts.tex <==

\section{No U-Turn Sampler}
\label{sec:nuts}

\mj{this is great but quite long. ideally this gets split into two sections: i) a short, compact section that gets across the main idea (iterative instead of recursive) and goes in the main text; and ii) a longer, technical description that goes into the appendix.}

	\subsection{Iterative NUTS sampler}
	
	\subsubsection{Motivation}
	
	The No-U-Turn Sampler \cite{hoffman2014no} is an extension of Hamiltonian Monte Carlo (HMC) that utilizes Hamiltonian dynamics to obtain samples from a target distribution $p(z)$. In HMC, an auxiliary momentum variable $r$ is used so that we can apply Hamiltonian dynamics on the combined state $(z, r)$. NUTS further utilizes the momentum variable to decide if the trajectory is making a U-turn. If it is the case, the process is terminated. Therefore, in NUTS, neither the trajectory length nor the number of leapfrog steps needs to be specified before hand. Usually, the length of each trajectory is a tuning parameter, which needs to be tuned for each specific problem, especially for high-dimensional or hierarchical models.
	
    %For each step, NUTS keeps doubling the current tree by creating a new tree with the same depth and merging two trees together. To construct a new tree with depth $d$, NUTS uses recursion as follows. We first build a left subtree, which has depth $d-1$. If this subtree is turning, the process stops there. Otherwise, a right subtree is built. If the right subtree is turning or the whole tree is tuning, stop. Otherwise, combine the left and the right subtrees together. And move to the next doubling step. The tail case of this recursion is when d = 0, which corresponds to a base tree collapsing to one single node.
    
    For each step, NUTS keeps doubling the current tree by creating a new tree with the same depth and merging two trees together. To construct a new tree with depth $d$, NUTS uses recursion as in \ref{alg:recursion}. This recursion process has both advantages and disadvantages. An advantage is its memory-friendliness because when combining two subtrees, we just need to store the information of the leftmost leaf of the left subtree and the rightmost leaf of the right subtree, so we don't need to store the information of middle leaves. Hence, memory requirements to build a tree with depth $d$ is only $O(d)$ even though it requires $2^d$ leapfrog steps. However, recursion prohibits compiling the whole program into machine codes.
	
	A temporary solution is to compile only a small part of the algorithm, in particular, a leapfrog step. However, to build a trajectory, we might need $O(2^d)$ leapfrog steps. So even if the overhead of each step is small, the accumulated one will be large. This issue motivates us to convert the recursive algorithm to an iterative one, which allows to compile the process of generating the whole trajectory, hence setting the overhead to minimum.
	
	\subsubsection{Method}
	
	To be able to compile the whole program using NUTS, we replace recursion by iteration. We will also keep the memory requirement linear in terms of the depth of the tree.
	
	Assume that we need to build a tree with depth $d$, we will construct $2^d$ leaves $z_0, \ldots, z_{2^d-1}$ iteratively but will stop when turning condition happens. First, we need to decide when to check for U-turn such that it is equivalent to the recursive algorithm.
	
	For that purpose, we use binary representation of the leaf index which gives its position in a binary tree without having to count indices from left to right. For example, in Figure \ref{fig:binary_rep}, we only need three steps to find the position of leaf $6=(110)_{2}$: start at the top of leftmost subtree with depth $3$ (the length of the binary representation), go down one level to the right (which corresponds to the first $1$ in the binary representation), then go down another level to the right (which corresponds to the next $1$ in the binary representation), and finally go down one level to the left (which corresponds to the $0$ in the binary representation). The idea behind is to focus on the depth axis instead of the index axis.

	\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{binary_rep.pdf}
	\caption{Example of finding the position of leaf $6=(110)_2$ on a binary tree. }
	\label{fig:binary_rep}
    \end{figure}

	For an index $n$, we denote by $\mathrm{B}(n, i)$ the $i$-th bit, counted from right to left, in the binary representation of $n$. In addition, we denote its depth-$k$ subtree by
	$$\mathrm{St}(n, k) = \left\{m \mid \mathrm{B}(m, i)= \mathrm{B}(n,i) \textrm{ for all } i \ge k \right\}.$$
	For example, 
	$$\mathrm{St}(6, 1) = \{(110)_{2}, (111)_{2}\} =\{6, 7\}.$$
	The leftmost leaf of the above depth-$k$ subtree is denoted by $\mathrm{St}(n, k, \textrm{left})$. In particular, 
	$$ \mathrm{B}(\mathrm{St}(n, k, \textrm{left}), i)=
	\begin{cases}\mathrm{B}(n,i) &\text{if } i \ge k, \\
	  0 &\text{if } i < k.
	\end{cases}$$

	
	Given an index $n$, we need to check the U-turn condition for all the subtrees whose rightmost leaf is $n$. Since the rightmost leaf of a depth-$k$ subtree contains only $1$ in the last $k$ bits, assume that the number of contiguous rightmost $1$ of $n$ is $l$, then the leftmost leaves of those subtrees for which we need to check the U-turn condition are precisely $\mathrm{St}(n, k, \textrm{left})$ for all $1\le k \le l$. For example, for $n=11$, the leftmost leaves for checking U-turn are nodes $0, 8,$ and $10$. Note that we have found these leaves by following the depth axis instead of the index axis.

	Now, recall that recursion algorithm is effective because its memory requirement is linear in terms of the depth of the tree. The trickiest issue that we have to deal with is to maintain the memory effectiveness of the recursion.

	To illustrate our strategy, let us start with a simple observation. For the tree in Firgure \ref{fig:binary_tree}, for all $n\ge 8$, among the nodes $0, 1, \dots, 7$ of the left subtree, only node $0$ ever occurs as a leftmost leaf for checking U-turn for any $n\ge 8$. We say that $0$ is a ``useful" leaf at $n=8$. More generally, a leaf is said to be a useful leaf at $n$ if it is used for checking U-turn for some node $m\ge n$. If a leaf $n$ is in the right subtree of a depth-$k$ subtree (in other words, $B(n, k - 1) = 1$), then the only useful leaf from the left subtree of $St(n, k)$ is $St(n, k, \textrm{left})$. In other words, at step $n$, the useful leaves are $\mathrm{St}(n,k,\textrm{left})$ for all $k$ at which $\mathrm{B}(n, k-1) = 1$. That leads us to Algorithm \ref{alg:iteration}, where we use the storage $R$ to save the useful leaves, update $R$ at even steps, and check U-turn condition to relevant leaves in $R$  at odd steps.
	
	
	
	\begin{figure}
		\centering
		\includegraphics[width=0.48\textwidth]{binary_tree.pdf}
		\caption{Example of constructing a binary tree using iteration. Orange node is the leaf generated at the current step. Blue nodes are the leaves stored in the memory for the purpose of checking U-turn condition. Green node is the proposal leaf of the current tree. White nodes are past leaves which have been removed from the memory. Dashed white nodes have not been generated yet. Black curves link the left leaf and right leaf of subtrees which we need to check if U-turn happens.}
		\label{fig:binary_tree}
	\end{figure}

	
	
%	For example, consider a tree of depth $d=3$. As seen in the above discussion, the maximum number of leftmost leaves to check for U-turn is at most $d$, we will need to store these nodes in a three-dimensional storage $R[0], R[1], R[2]$. Assume that the current node is at $n=10=(1010)_2$, then its number of 1-bits, $\mathrm{bitcount}(10)$, is $2$. We set $R[2] = \textrm{leaf } 10$. At step $11 = (1011)_2$, we need to check U-turn condition with leaf $(1000)_2 = R[1]$ and leaf $(1010)_2 = R[2]$. At step $12 = (1100)_2$, because $\mathrm{bitcount}(12) = 2$, we set $R[2] = \textrm{leaf } 12$, in other words, at this step, node $10$ is not required anymore.


	\begin{minipage}{0.48\textwidth}
	\begin{algorithm}[H]
		\caption{Build a Tree using Recursion}
		\label{alg:recursion}
		\begin{algorithmic}
			\STATE {\bfseries function} {BuildTree}(initial node $z$, depth $d$)
			\IF{$d = 0$}
			\STATE $z_{new} \leftarrow \mathrm{Leapfrog}(z)$
			\STATE $left \leftarrow z_{new}$
			\STATE $right \leftarrow z_{new}$
			\STATE $turning \leftarrow False$
			\STATE {\bfseries returns} $\mathrm{Tree}(left, right, turning)$
			\ELSE
			\STATE $leftTree = \mathrm{BuildTree}(z_{-1}, d - 1)$
			\IF{$leftTree.turning$}
			\STATE {\bfseries returns} $leftTree$
			\ENDIF
			\STATE $z \leftarrow leftTree.right$
			\STATE $rightTree \leftarrow \mathrm{BuildTree}(z, d - 1)$
			\STATE $left \leftarrow leftTree.left$
			\STATE $right \leftarrow rightTree.right$
			\IF{$rightTree.turning$}
			\STATE $turning = True$
			\ELSE
			\STATE $turning \leftarrow \mathrm{CheckUTurn}(left, right)$
			\ENDIF
			\STATE {\bfseries returns} $\mathrm{Tree}(left, right, turning)$
			\ENDIF
		\end{algorithmic}
	\end{algorithm}
	\end{minipage}
	\hfill
	\begin{minipage}{0.48\textwidth}
	\begin{algorithm}[H]
		\caption{Build a Tree using Iteration}
		\label{alg:iteration}
		\begin{algorithmic}
			\STATE {\bfseries Input:} initial node $z_{-1}$, depth $d$
			\STATE {\bfseries Initialize:} storage $R[0], R[1], \dots, R[d-1]$
			\STATE $n \leftarrow -1$
			\STATE $turning \leftarrow False$ 
			\WHILE{$n < 2^d - 1$ \AND not $turning$}
			\STATE $n \leftarrow n + 1$
			\STATE $z_n \leftarrow \mathrm{Leapfrog}(z_{n-1})$
			\IF{$n$ is even}
			\STATE $i \leftarrow \mathrm{bitcount}(n)$
			\STATE $R[i] \leftarrow z_n$
			\ELSE[$n$ is odd]
			\STATE $i_{max} \leftarrow \mathrm{bitcount}(n-1)$
			\STATE // number of last contiguous 1-bits
			\STATE $l = \mathrm{bitcount}(((n + 1) \mathbin{\&} \ensuremath{\mathord{\sim}} n) - 1)$
			\STATE $i_{min} = i_{max} - l + 1$
			\FOR{$k=i_{max}$ {\bfseries to} $i_{min}$}
			\STATE $turning \leftarrow \mathrm{CheckUTurn}(R[k], z_n)$
			\IF{$turning$}
			\STATE {\bfseries break}
			\ENDIF
			\ENDFOR
			\ENDIF
			\ENDWHILE
			\STATE {\bfseries returns} $z_0$, $z_n$, $turning$
		\end{algorithmic}
	\end{algorithm}
	\end{minipage}
	
	Having addressed the memory effectiveness, we succeed in converting recursive nature of NUTS to an iterative one. The iterative scheme allows more control on the process; for example, it might allow adding more stopping conditions to the scheme. The biggest advantage right now is that it allows to compile the computation of the whole trajectory thereby hugely reducing the overhead cost.
	
		\subsubsection{Implementation}
	
	Note that in Algorithm \ref{alg:iteration}, given $n$, indices $i$, $i_{min}$, $i_{max}$ of the storage $R$ only requires $\mathrm{bitcount}$ operators, which is pretty cheap to compute. We can create a table of those indices given $n$ but we found that it is not necessary.
	
	Since original implementation of NUTS, we use generalized termination criterion and replace slice sampling by multinomial sampling following \cite{betancourt2017conceptual}.
	
	To draw multiple chains, we provide several options: "parallel", "sequential", "vectorized". The method 'parallel' is used to execute the drawing process in parallel on XLA devices (CPUs/GPUs/TPUs). If there are not enough devices for 'parallel', we fall back to 'sequential' method to draw chains sequentially. 'vectorized' method is an experimental feature which vectorizes the drawing method, hence allows us collecting samples in parallel on a single device. All experiments in Experiments section are done using 'parallel' method.

==> nuts_rev1.tex <==

\section{No U-Turn Sampler}
\label{sec:nuts}
	No-U-Turn Sampler (NUTS) \cite{JMLR:v15:hoffman14a} is an extension of Hamiltonian Monte Carlo (HMC) algorithm, which can efficiently sample from high-dimensional continuous probability distributions. NUTS adaptively sets the trajectory length parameter in HMC, which along with the adaptation of the step size and mass matrix parameters, ensures that HMC runs efficiently on a variety of models without any hand-tuning involved. This provides a highly attractive black-box inference algorithm for PPLs to have in their toolkit. 
	
\subsection{Iterative NUTS}
Existing NUTS implementations use a recursive tree building formulation as discussed in \citet[Algorithm 6]{JMLR:v15:hoffman14a}. Computing a trajectory in NUTS involves a doubling procedure where at each iteration, we run the LeapFrog integrator for double the number of steps in the forward or reverse direction randomly, which has the effect of building an implicit balanced binary tree. The doubling process is terminated when a subtrajectory from the leftmost to the rightmost node of any balanced subtree begins to double back on itself. 

A key component of this algorithm is the recursive \verb|BuildTree| procedure. To build a tree at depth $d$, it builds two subtrees at depth $d-1$ and combines them. This recursive procedure also takes care to ensure that the memory consumption scales as $\mathcal{O}(\log{}n)$ ($\mathcal{O}(d)$) rather than $\mathcal{O}(n)$ by only storing $\mathcal{O}(1)$ information per subtree. This is important because storing all $n$ momentum-position pairs might be prohibitive for large models. However, the recursive solution is not amenable to JIT compilation [todo: mention limitation] in JAX. This was also noticed by \citet{tran2018simple} for Edward2 which runs TensorFlow in Eager mode for NUTS. An alternative would be to JIT compile a single LeapFrog step or the potential energy function (the latter being followed in Pyro's NUTS implementation), but drawing a single sample involves many LeapFrog steps and the overhead in terms of Python function dispatch calls is significant. More importantly, this also takes away any opportunities for XLA operation fusion. This motivated our work on an iterative version of the NUTS algorithm that can be fully JIT compiled. In particular, this involves converting the \verb|BuildTree| procedure into an iterative procedure, paving the way to JIT compile NUTS sampling.

\subsection{Algorithm Details}

The iterative version of NUTS takes an initial node (position-momentum pair) $z_{-1}$ and a depth $d$ argument, and runs the LeapFrog integrator for $n=2^d$ steps. We will be using 0 based indexing, and nodes in the new tree constructed by iterative \verb|BuildTree| are numbered starting from 0. Assume that $b(n)$ is the binary representation of the node $z_n$. Then for $z_n$, we need to check the U-Turn condition with respect to the leftmost nodes of any binary subtree for which $z_n$ is the rightmost node. This is given by candidates whose binary representation is the same as $n$ except that trailing contiguous 1s in $b(n)$ are progressively masked by 0 (see Algorithm~ \ref{alg:candidate-set}). e.g. The binary representation for $11$ is $(1011)_2$, and the set of candidate nodes for checking the U-Turn condition are given by ${(1010)_2, (1000)_2} = {8, 10}$. Note that this implies that we can skip checks at even numbered nodes.

This allows us to iteratively build the binary tree by running the LeapFrog integrator for $2^d$ steps, and terminating early if the U-Turn condition stated above is satisfied. However, we would naively still need $O(n)$ memory since we will have to store the position-momentum pair at each step of the integrator, which is a far cry from the $\mathcal{O}(\log{}n)$ memory requirement of the recursive solution. To tackle the question of memory efficiency, we claim that we can use an array $S$ of size $d$ to store the node data when $n$ is even at index \verb|BitCount(n)|. The data for the candidate nodes must be present in $S$ because the nodes in \verb|CandidateSet(n)| are the largest nodes less than $n$ for that bit count. Full details of the algorithm are provided in Algorithm~\ref{alg:iterative-nuts}.

\begin{figure}
\begin{minipage}[t]{0.52\textwidth}
\begin{algorithm}[H]
  \caption{\textsc{IterativeBuildTree}}
  \label{alg:iterative-nuts}
  {\bf Input} initial node $z_{-1}$ \\
  \phantom{\bf Input} tree depth $d$ \\
  {\bf Initialize} storage $S[0], S[1], ..., S[d-1]$ \\
    \phantom{\bf Initialize} $ n \from {-1}$ \\
    \phantom{\bf Initialize} $ turning \from False$\\
  \While{$n < 2^d$ \textrm{\bf{and not}} $turning$}{
    $z_{n+1} \from \mathrm{\textsc{Leapfrog}}(z_n)$ \\
    $n \from n+1$ \\
    \eIf{$n$ is even}{
      $ i \from \mathrm{\textsc{BitCount}}(n) $ \\
      $S[i] \from z_n$
    }{
      $c \from \textrm{\textsc{CandidateSet}}(n)$ \\
      \While{\textrm{\bf not} c.empty()}{
        $k \from \textrm{\textsc{BitCount}}(c.pop())$ \\
        $turning \from \textrm{\textsc{CheckUTurn}}(S[k], z_n)$ \\
        \If{turning}{
          \textbf{break}
        }
      }
    }
  }
\Return $z_n, turning$ \\
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\textwidth}
\begin{algorithm}[H]
  \caption{\textsc{CandidateSet}}
  \label{alg:candidate-set}
  {\bf Input} node index $n$ \\
  {\bf Initialize} $S \from [] $ \\
  // Number of last contiguous 1s \\
  $j \from \textrm{\textsc{BitCount}}((n+1) \& \sim n - 1) $ \\
  \For{$k$ = 1 \textrm{\bf to} j}{
    // progressively mask trailing 1s with 0s
    $m \from \ \sim((1 << k) - 1) $ \\
    S.push($n \& m$) 
  }
\Return S
\end{algorithm}
\end{minipage}
\caption{The \texttt{IterativeBuildTree} algorithm. Note that this is a simplified version of the actual algorithm which needs to store (and return) additional metadata in \texttt{S} such as the proposal candidate. This also does not consider other inputs to the function such as the step size and the direction, which are not relevant to the changes proposed.}
\end{figure}


==> nuts_short.tex <==

\section{No U-Turn Sampler}
\label{nuts}

	\subsection{Iterative NUTS sampler}
	
	\subsubsection{Motivation}
	
	No-U-Turn Sampler is an extension of Hamiltonian Monte Carlo (HMC) which utilizes Hamiltonian dynamics to obtain samples from a target distribution $p(z)$. In HMC, an auxiliary momentum variable $r$ is used so that we can apply Hamiltonian dynamics on the combined state $(z, r)$. NUTS further utilizes the momentum variable to decide if the trajectory is making a U-turn. If it is the case, the process is terminated. Therefore, in NUTS, neither the trajectory length nor the number of leapfrog steps needs to be specified before hand. Usually, the length of each trajectory is a tuning parameter, which needs to be tuned for each specific problem, especially for high dimensional or hierarchy models.
	
    %For each step, NUTS keeps doubling the current tree by creating a new tree with the same depth and merging two trees together. To construct a new tree with depth $d$, NUTS uses recursion as follows. We first build a left subtree, which has depth $d-1$. If this subtree is turning, the process stops there. Otherwise, a right subtree is built. If the right subtree is turning or the whole tree is tuning, stop. Otherwise, combine the left and the right subtrees together. And move to the next doubling step. The tail case of this recursion is when d = 0, which corresponds to a base tree collapsing to one single node.
    
    For each step, NUTS keeps doubling the current tree by creating a new tree with the same depth and merging two trees together. To construct a new tree with depth $d$, NUTS uses recursion as in Algorithm \ref{alg:recursion}. This recursion process has both advantages and disadvantages. An advantage is its memory-friendliness because when combining two subtrees, we just need to store the information of the leftmost leaf of the left subtree and the rightmost leaf of the right subtree, so we don't need to store the information of middle leaves. Hence, memory requirements to build a tree with depth $d$ is only $O(d)$ even though it requires $2^d$ leapfrog steps. However, recursion prohibits compiling the whole program into machine codes.
	
	A temporary solution is to compile only a small part of the algorithm, in particular, a leapfrog step. However, to build a trajectory, we might need $O(2^d)$ leapfrog steps. So even if the overhead of each step is small, the accumulated one will be large (see e.g. \cite{tran2018simple}), especially when a lot of samples are needed. This issue motivates us to convert the recursive algorithm to an iterative one, which allows to compile the process of generating the whole trajectory, hence setting the overhead to minimum.
	
	\subsubsection{Method}
	
	To be able to compile the whole program using NUTS, we replace recursion by iteration. We will also keep the memory requirement linear in terms of the depth of the tree.
	
	Assume that we need to build a tree with depth $d$, we will construct $2^d$ leaves $z_0, \ldots, z_{2^d-1}$ iteratively but will stop when turning condition happens. First, we need to decide when to check for U-turn such that it is equivalent to the recursive algorithm.
	
	For that purpose, we use binary representation of the leaf index which gives its position in a binary tree without having to count indices from left to right. For example, in Figure \ref{fig:binary_rep}, we only need three steps to find the position of leaf $6=(110)_{2}$: start at the top of leftmost subtree with depth $3$ (the length of the binary representation), go down one level to the right (which corresponds to the first $1$ in the binary representation), then go down another level to the right (which corresponds to the next $1$ in the binary representation), and finally go down one level to the left (which corresponds to the $0$ in the binary representation). The idea behind is to focus on the depth axis instead of the index axis.

	\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{binary_rep.pdf}
	\caption{Example of finding the position of leaf $6=(110)_2$ on a binary tree. }
	\label{fig:binary_rep}
    \end{figure}

	For an index $n$, we denote by $\mathrm{B}(n, i)$ the $i$-th bit, counted from right to left, in the binary representation of $n$. In addition, we denote its depth-$k$ subtree by
	$$\mathrm{St}(n, k) = \left\{m \mid \mathrm{B}(m, i)= \mathrm{B}(n,i) \textrm{ for all } i \ge k \right\}.$$
	For example, 
	$$\mathrm{St}(6, 1) = \{(110)_{2}, (111)_{2}\} =\{6, 7\}.$$
	The leftmost leaf of the above depth-$k$ subtree is denoted by $\mathrm{St}(n, k, \textrm{left})$. In particular, 
	$$ \mathrm{B}(\mathrm{St}(n, k, \textrm{left}), i)=
	\begin{cases}\mathrm{B}(n,i) &\text{if } i \ge k, \\
	  0 &\text{if } i < k.
	\end{cases}$$

	
	Given an index $n$, we need to check the U-turn condition for all the subtrees whose rightmost leaf is $n$. Since the rightmost leaf of a depth-$k$ subtree contains only $1$ in the last $k$ bits, assume that the number of contiguous rightmost $1$ of $n$ is $l$, then the leftmost leaves of those subtrees for which we need to check the U-turn condition are precisely $\mathrm{St}(n, k, \textrm{left})$ for all $1\le k \le l$. For example, for $n=11$, the leftmost leaves for checking U-turn are nodes $0, 8,$ and $10$. Note that we have found these leaves by following the depth axis instead of the index axis.

	Now, recall that recursion algorithm is effective because its memory requirement is linear in terms of the depth of the tree. The trickiest issue that we have to deal with is to maintain the memory effectiveness of the recursion.

	To illustrate our strategy, let us start with a simple observation. For the tree in Firgure \ref{fig:binary_tree}, for all $n\ge 8$, among the nodes $0, 1, \dots, 7$ of the left subtree, only node $0$ ever occurs as a leftmost leaf for checking U-turn for any $n\ge 8$. We say that $0$ is a ``useful" leaf at $n=8$. More generally, a leaf is said to be a useful leaf at $n$ if it is used for checking U-turn for some node $m\ge n$. If a leaf $n$ is in the right subtree of a depth-$k$ subtree (in other words, $B(n, k - 1) = 1$), then the only useful leaf from the left subtree of $St(n, k)$ is $St(n, k, \textrm{left})$. In other words, at step $n$, the useful leaves are $\mathrm{St}(n,k,\textrm{left})$ for all $k$ at which $\mathrm{B}(n, k-1) = 1$. That leads us to Algorithm \ref{alg:iteration}, where we use the storage $R$ to save the useful leaves, update $R$ at even steps, and check U-turn condition to relevant leaves in $R$  at odd steps.
	
	
	
	\begin{figure}
		\centering
		\includegraphics[width=0.90\textwidth]{binary_tree.pdf}
		\caption{Example of constructing a binary tree using iteration. Orange node is the leaf generated at the current step. Blue nodes are the leaves stored in the memory for the purpose of checking U-turn condition. Green node is the proposal leaf of the current tree. White nodes are past leaves which have been removed from the memory. Dashed white nodes have not been generated yet. Black curves link the left leaf and right leaf of subtrees which we need to check if U-turn happens.}
		\label{fig:binary_tree}
	\end{figure}

	
	
%	For example, consider a tree of depth $d=3$. As seen in the above discussion, the maximum number of leftmost leaves to check for U-turn is at most $d$, we will need to store these nodes in a three-dimensional storage $R[0], R[1], R[2]$. Assume that the current node is at $n=10=(1010)_2$, then its number of 1-bits, $\mathrm{bitcount}(10)$, is $2$. We set $R[2] = \textrm{leaf } 10$. At step $11 = (1011)_2$, we need to check U-turn condition with leaf $(1000)_2 = R[1]$ and leaf $(1010)_2 = R[2]$. At step $12 = (1100)_2$, because $\mathrm{bitcount}(12) = 2$, we set $R[2] = \textrm{leaf } 12$, in other words, at this step, node $10$ is not required anymore.

	\begin{minipage}{0.49\textwidth}
	\begin{algorithm}[H]
		\caption{\textsc{BuildTree}}
		\label{alg:recursion}
		{\bf Input} initial node $z$ \\
		\phantom{\bf Input} tree depth $d$ \\
		\eIf{$d = 0$}{
			$z_{new} \from \mathrm{\textsc{Leapfrog}}(z)$ \\
			\Return $\mathrm{\textsc{Tree}}(z_{new}, z_{new}, False)$
		}{
			$left\_tree \from \mathrm{\textsc{BuildTree}}(z, d - 1)$ \\
			\eIf{$left\_tree.turning$}{
				\Return $left\_tree$
			}{
				$z \from left\_tree.right$ \\
				$right\_tree \from \mathrm{\textsc{BuildTree}}(z, d - 1)$ \\
				$l \from left\_tree.left$ \\
				$r \from right\_tree.right$ \\
				\eIf{$right\_tree.turning$}{
					$turn \from True$
				}{
					$turn \from \textrm{\textsc{CheckUTurn}}(l, r)$
				}
				\Return $\mathrm{\textsc{Tree}}(l, r, turn)$
			}
		}
	\end{algorithm}
	\end{minipage}
	\hfill
	\begin{minipage}{0.49\textwidth}
	\begin{algorithm}[H]
	\caption{\textsc{IterativeBuildTree}}
	\label{alg:iteration}
		{\bf Input} initial node $z$ \\
		\phantom{\bf Input} tree depth $d$ \\
		{\bf Initialize} storage $S[0], S[1], ..., S[d-1]$ \\
		\For{$n \from 0$ \KwTo $2^d - 1$}{
			$z \from \mathrm{\textsc{Leapfrog}}(z)$ \\
			\eIf{$n$ is even}{
				$ i \from \mathrm{\textsc{BitCount}}(n) $ \\
				$S[i] \from z$
			}{
				$ i_{max} \from \mathrm{\textsc{BitCount}}(n) - 1 $ \\
				// number of last contiguous 1-bits of $n$ \\
				$l \from \textrm{\textsc{BitCount}}(((n + 1) \mathbin{\&} \ensuremath{\mathord{\sim}} n) - 1)$ \\
				$i_{min} \from i_{max} - l + 1$ \\
				\For{$k \from i_{max}$ \KwTo $i_{min}$}{
					$turn \leftarrow \mathrm{\textsc{CheckUTurn}}(S[k], z)$  \\
					\If{turn}{
						\Return $\mathrm{\textsc{Tree}}(S[0], z, True)$
					}
				}
			}
		}
		\Return $\mathrm{\textsc{Tree}}(S[0], z, False)$
	\end{algorithm}
	\end{minipage}
	
	Having addressed the memory effectiveness, we succeed in converting recursive nature of NUTS to an iterative one. The iterative scheme allows more control on the process; for example, it might allow adding more stopping conditions to the scheme. The biggest advantage right now is that it allows to compile the computation of the whole trajectory thereby hugely reducing the overhead cost.
	
		\subsubsection{Implementation}
	
	Note that in Algorithm \ref{alg:iteration}, given $n$, indices $i$, $i_{min}$, $i_{max}$ of the storage $R$ only requires $\mathrm{bitcount}$ operators, which is pretty cheap to compute. We can create a table of those indices given $n$ but we found that it is not necessary.
	
	Since original implementation of NUTS, we use generalized termination criterion and replace slice sampling by multinomial sampling following \cite{betancourt2017conceptual}.
	
	To draw multiple chains, we provide several options: "parallel", "sequential", "vectorized". The method 'parallel' is used to execute the drawing process in parallel on XLA devices (CPUs/GPUs/TPUs). If there are not enough devices for 'parallel', we fall back to 'sequential' method to draw chains sequentially. 'vectorized' method is an experimental feature which vectorizes the drawing method, hence allows us collecting samples in parallel on a single device. All experiments in Experiments section are done using 'parallel' method.
